Next-to-Leading Order QCD Predictions for Z,gamma^*+3-Jet Distributions at the Tevatron

Using BlackHat in conjunction with SHERPA, we have computed next-to-leading order QCD predictions for a variety of distributions in Z,gamma*+1,2,3-jet production at the Tevatron, where the Z boson or off-shell photon decays into an electron-positron pair. We find good agreement between the NLO results for jet p_T distributions and measurements by CDF and D0. We also present jet-production ratios, or probabilities of finding one additional jet. As a function of vector-boson p_T, the ratios have distinctive features which we describe in terms of a simple model capturing leading logarithms and phase-space and parton-distribution-function suppression.

==> figs/darkengray <==
#!/bin/csh -f

cp $1 darkgrey_tmp1.eps
cp $1 $1_bak

sed s/Color7" "\{0.8627" "0.8627" "0.8627\}/Color7" "\{0.6" "0.6" "0.6\}/ darkgrey_tmp1.eps > darkgrey_tmp2.eps
sed s/Color11" "\{1.0000" "0.6471" "0.0000\}/Color11" "\{.7" ".4" "0.\}/ darkgrey_tmp2.eps > darkgrey_tmp3.eps 

cp darkgrey_tmp3.eps $1
rm -f darkgrey_tmp1.eps
rm -f darkgrey_tmp2.eps
rm -f darkgrey_tmp3.eps

